The Hierarchical Structure of Galactic Haloes: Differentiating Clusters from Stochastic Clumping with AstroLink

We present AstroLink, an efficient and versatile clustering algorithm designed to hierarchically classify astrophysically-relevant structures from both synthetic and observational data sets. We build upon CluSTAR-ND, a hierarchical galaxy/(sub)halo finder, so that AstroLink now generates a two-dimensional representation of the implicit clustering structure as well as ensuring that clusters are statistically distinct from the noisy density fluctuations implicit within the $n$-dimensional input data. This redesign replaces the three cluster extraction parameters from CluSTAR-ND with a single parameter, $S$ -- the lower statistical significance threshold of clusters, which can be automatically and reliably estimated via a dynamical model-fitting process. We demonstrate the robustness of this approach compared to AstroLink's predecessors by applying each algorithm to a suite of simulated galaxies defined over various feature spaces. We find that AstroLink delivers a more powerful clustering performance while being $\sim27\%$ faster and using less memory than CluSTAR-ND. With these improvements, AstroLink is ideally suited to extracting a meaningful set of hierarchical and arbitrarily-shaped astrophysical clusters from both synthetic and observational data sets -- lending itself as a great tool for morphological decomposition within the context of hierarchical structure formation.

==> aggregate.tex <==
\begin{figure}
\begin{center}
\begin{tikzpicture}[node distance=1.5cm, every node/.style={fill=white, text centered, font=\sffamily}], align=center]
    % Specification of nodes (position, etc.)
    \node[align = center] (input)[base]
    {Input the points ($P$), the $k_\mathrm{den}$ nearest\\neighbours ($N_{k_\mathrm{den}}$), and the scaled log-densities ($\log\hat{\rho}$).};
    
    \node[align = center] (reduce_neighbours)[base, below of=input]
    {Find $p_i$'s $k_\mathrm{link}$ nearest neighbours ($N_{k_\mathrm{link},i} \subseteq N_{k_\mathrm{den},i}$) $\forall p_i \in P$.};
    
    \node[align = center] (compute_edges)[base, below of=reduce_neighbours]
    {Compute the set of edges $E$, where\\$E_{ij} = \mathrm{min}\{\log\hat{\rho}_i,\ \log\hat{\rho}_j\}$, $\forall p_i \in P \land \forall p_j \in N_{k_\mathrm{link},i}$.};

    \node[align = center] (initialise_sets)[base, below of=compute_edges]
    {Initialise the empty sets; $A = \varnothing$, $G_\leq = \varnothing$, and $G_\geq = \varnothing$.};




    
    \node[align = center] (next_point)[repeat1, below of=initialise_sets, xshift = -0.5cm]
    {Retrieve points, $p_i$ and $p_j$, such that $E_{ij} = \mathrm{max}\ E$.\\Remove $E_{ij}$ from $E$.};
    
    \node[align = center] (connections)[repeat1, below of=next_point]
    {Find $A_i \in A$ and $A_j \in A$, such that\\$p_i \in A_i$ (or $A_i = \varnothing$) and $p_j \in A_j$ (or $A_j = \varnothing$).};
    
    
    
    
    \node(if_both_not_aggregated)[text width = 2cm, below of=connections, xshift=-2.25cm]
    {if $A_i = A_j = \varnothing$};

    \node[align = center] (new_aggregation)[repeat2, below of=connections, xshift=1.2cm, minimum width = 3.5cm]
    {Add $\{p_i, p_j\}$ ($\{p_j, p_i\}$)\\to $A$ if $\log\hat{\rho}_i \geq (<) \log\hat{\rho}_j$.};
    
    \node(if_same_group)[text width = 2cm, below of=if_both_not_aggregated, yshift=0.5cm]
    {if $A_i = A_j \neq \varnothing$};

    \node(if_one_not_aggregated)[text width = 2.3cm, below of=if_same_group, yshift=0.5cm]
    {if $A_i = \varnothing \lor A_j = \varnothing$};

    \node[align = center] (append)[repeat2, below of=new_aggregation, yshift=-0.5cm, minimum width = 3.5cm]
    {Add $p_j$ ($p_i$) to $A_i$ ($A_j$)\\if $A_j (A_i) = \varnothing$.};

    \node[align = center] (join)[repeat2, below of=append, xshift=-1.475cm, minimum width = 6.45cm]
    {Add $A_<$ to $G$ and $A_\geq$ to $G_\mathrm{comp}$.\\Remove $A_<$ from $A$ and add it to $A_\geq$.};


    
    \node[align = center] (while_u)[repeat1, below of=connections, xshift = 4cm, yshift = -1.75cm, rotate=-90, minimum width = 4.5cm]
    {While $E \neq \varnothing$};
    
    
    
    

    \node[align = center] (merge_forest)[base, below of=join, xshift = 0.775cm]
    {Remove the largest element of $A$ and call it $O$.\\Then $\forall A_i \in A$; add $A_i$ to $G$, $O$ to $G_\mathrm{comp}$, and then $A_i$ to $O$.};
    
    \node[align = center] (output)[base, below of=merge_forest]
    {Output the ordered list ($O$), $P$'s subgroups ($G$),\\and $G$'s complementary groups ($G_\mathrm{comp}$).};
    
    % Specification of lines between nodes specified above
    % with additional nodes for description
    \draw[->](input) -- (reduce_neighbours);
    \draw[->](reduce_neighbours) -- (compute_edges);
    \draw[->](compute_edges) -- (initialise_sets);
    \draw[->](initialise_sets) -- +(0, -1);
    \draw[->](next_point) -- (connections);
    \draw[<-](if_both_not_aggregated) -- +(0, 1);
    \draw[->](if_both_not_aggregated) -- (new_aggregation);
    \draw[->](new_aggregation.east) -- +(0.5, 0);
    \draw[<-, dashed](if_same_group) -- +(0, 0.75);
    \draw[->](if_same_group) -- +(5.75, 0);
    \draw[<-, dashed](if_one_not_aggregated) -- +(0, 0.75);
    \draw[->](if_one_not_aggregated) -- (append);
    \draw[->](append.east) -- +(0.5, 0);
    \draw[->, dashed](if_one_not_aggregated) -- +(0, -1);
    \draw[->](join.east) -- +(0.5, 0);
    \draw[->](while_u) |- (next_point);
    \draw[->, dashed](while_u.east) -- +(0, -0.5);
    \draw[->](merge_forest) -- (output);
\end{tikzpicture}
\end{center}
\vspace{-4pt}
\caption{Activity chart for \astrolink's improved aggregation process that constructs the hierarchy of subgroups and there complementary groups, as well as a point ordering analogous to the \optics\ reachability plot. First, the $k_\mathrm{den}$ nearest neighbour lists are reduced to $k_\mathrm{link}$ and the edges $E$ are computed. The edges are then used to manipulate the active aggregations ($A$) by initiating new aggregations, adding points to existing aggregations, or merging existing aggregations and adding to $P$'s subgroups ($G$) and their complementary groups $G_\mathrm{comp}$. Following this, remaining active aggregations are added to $G$ (except the largest) and concatenated to form the ordered point list $O$. The function, $f(i) = \log\hat{\rho}_i,\ \forall i \in O$, serves as \astrolink's equivalent of the \optics\ reachability plot (shown in Fig. \ref{fig:agg_example}), and the subgroup and complementary group hierarchy is represented by $g \in G$ and $g_\mathrm{comp} \in G_\mathrm{comp}$ and their corresponding merger tree (shown in Fig. \ref{fig:merg_example}).}
\label{fig:aggregate}
\end{figure}

==> alg_wrapper.tex <==
\begin{figure}
\begin{center}
\begin{tikzpicture}[node distance=1.5cm, every node/.style={fill=white, text centered, font=\sffamily}], align=center]
    % Specification of nodes (position, etc.)
    \node[align = center] (input)[base]
    {Input the data and parameters.};
    
    \node[align = center] (fieldhaloes)[base, below of=input]
    {Find all field haloes using 3D \code{FOF} or treat\\input data as if it were a field halo.};
    
    \node[align = center] (searchforsubstructure)[base, below of=fieldhaloes]
    {For each field halo, search for substructure\\within it using the process in Fig. \ref{fig:searchsubstructure}.};
    
    \node[align = center] (output)[base, below of=searchforsubstructure]
    {Output the hierarchy of clusters.};
    
    % Specification of lines between nodes specified above
    % with additional nodes for description
    \draw[->](input) -- (fieldhaloes);
    \draw[->](fieldhaloes) -- (searchforsubstructure);
    \draw[->](searchforsubstructure) -- (output);
\end{tikzpicture}
\end{center}
\vspace{-8pt}
\caption{An activity of the outer methods of both the \clustar\ and \astrolink\ algorithms. Before finding the substructure each algorithm first decides on the root-level clusters - where the option is given to produce 3D \code{FOF} field haloes or to treat the input data as if it were a field halo. For \astrolink, the cluster search is completed once the process in Fig. \ref{fig:searchsubstructure} is finished for each field halo.}
\label{fig:rootlevel}
\end{figure}

==> fitting_example.tex <==
\begin{figure}
    \centering
    \includegraphics[trim={13.5mm 24mm 11mm 36mm}, clip, width=\columnwidth]{Images/fitting_example_compound_models.png}
    \vspace{-0.5cm}
    \caption{Example distributions of subgroup prominences that \astrolink\ produces (when $k_\mathrm{den} = 20$ and $adaptive = 0$) from various $n$-point $d$-dimensional data sets that have each been sampled from a uniform distribution defined over the volume of the unit hypercube. The different distribution models (a linear combination of the distributions \ref{dist:i} -- \ref{dist:v} and a uniform distribution) are shown fitted to this data in the way described in Sec. \ref{subsubsec:fitting}. Visually, each noise model could be considered a reasonable choice and as such it is not immediately obvious which is best.}
    \label{fig:fitting_example}
\end{figure}

==> full_merger_example.tex <==
\begin{figure}
    \centering
    \includegraphics[trim={13.5mm 1mm 11mm 9.5mm}, clip, width=\columnwidth]{Images/full_merger_example.png}
    \vspace{-0.5cm}
    \caption{A hypothetical example of a \textit{complete} merger tree and the corresponding prominence distribution that would occur when clustering over the same input data as is used in Figs. \ref{fig:merg_example} \& \ref{fig:prom_dist_example}. We can see here that if \astrolink\ were made to keep track of the largest group in every merger, the prominence distribution would become comparatively heavier in its tails and make the detection of clusters more difficult given that they would then present as less significant outliers in this distribution. Even though the clusters would still be detectable as outliers in the prominence distribution shown here, for other highly structured data sets this will not always be the case.}
    \label{fig:full_merg_example}
\end{figure}

==> parameter_table.tex <==
\begin{table*}
\centering
\caption{A short summary of the \astrolink\ inputs that are relevant to its clustering behaviour. \astrolink\ has a total of $6$ parameters, as opposed to the $7$ parameters of its predecessor \clustar, and for most clustering purposes it is only the choice of $l_x$, $adaptive$, $k_\mathrm{den}$, and $S$ that need to be considered. However, deciding their value is mostly a simple task. $l_x$ should only be set to a value other than $\infty$ when the user wishes for the root-level clusters to be defined by $3$D \code{FOF} groups -- a common definition for galaxies in cosmological simulation. $adaptive$ should only be set to $0$ when the features of the data have the same units or when a meaningful transform has been applied to the data prior to its input to \astrolink. $k_\mathrm{den}$ should be chosen according to the resolution of structure that the user wishes to find -- although a small value such as $k_\mathrm{den}$ was shown to produce the best clustering results in \citet{Oliver2022}. $S$ should be chosen to represent the strictness of confidence in the resulting clusters -- the clustering power over synthetic galaxies is shown as a function of $S$ in Fig. \red{XX}.}
\begin{tabular}{|c|c|c|c|}
\hline
Input & Default Value & Valid Values & Functionality \\
\hline
$P$ & --- & $n\times d$ array & The input data.\\
\hline
$adaptive$ & $1$ & $\{0, 1\}$ & A flag to apply a PCA transformation to field halo data. Refer to Sec. \ref{subsec:transformation} for more details.\\
\hline
$k_\mathrm{den}$ & $20$ & $\mathbb{N}_{\geq k_\mathrm{link}}$ & The number of nearest neighbours used to estimate local density. Refer to Sec. \ref{subsec:density_estimation} for more details. \\
\hline
$k_\mathrm{link}$ & $auto$ & $\mathbb{N}_{\geq 2 \land \leq k_\mathrm{den}}$ & The number of nearest neighbours used to aggregate points. Refer to Sec. \ref{subsubsec:connectivity} for more details. \\
\hline
$S$ & $5$ & $\mathbb{R}$ & The minimum statistical significance of extracted clusters. Refer to Sec. \ref{subsubsec:significance} for more details. \\
\hline
$h\_style$ & $1$ & $\{0, 1\}$ & A flag denoting the style of the extracted hierarchy. Refer to Sec. \ref{subsubsec:correction} for more details. \\
\hline
$workers$ & $-1$ & $\mathbb{N}_{\geq 0 \land \leq N_\mathrm{cpu}} \land \{-1\}$ & The number of cpu cores used to perform parallel processes. A value of $-1$ invokes using all cores.\\
\hline
$verbose$ & $2$ & $\mathbb{N}_{\geq 0}$ & The setting for the verbosity of the algorithm while it runs.\\
\hline
\end{tabular}
\label{tab:parameters}
\end{table*}

==> prominence_example.tex <==
\begin{figure}
    \centering
    \includegraphics[trim={13.5mm 1mm 11mm 9.5mm}, clip, width=\columnwidth]{Images/prominence_example.png}
    \vspace{-0.5cm}
    \caption{An example of how the calculation of the prominence ($\mathcal{P}$) relates to the ordered-density plot for the largest subgroup featured in Fig. \ref{fig:merg_example}. The $1$-dimensional Gaussian distribution that this subgroup represents only has small density fluctuations within it and as such is not penalised heavily by the $\log\hat{\rho}_{\mathrm{noise}, g}$ term. Refer to Sec. \ref{subsec:prominence} and Eq. \ref{eq:prominence} for more details on this calculation.}
    \label{fig:prominence_example}
\end{figure}

==> relative_likelihood.tex <==
\begin{figure}
    \centering
    \includegraphics[trim={11mm 1mm 11mm 9.5mm}, clip, width=\columnwidth]{Images/compound_model_relative_likelihood.png}
    \vspace{-0.5cm}
    \caption{The distributions of the relative likelihoods of the models outlined in Sec. \ref{subsubsec:prominencemodel}. The relative likelihoods have been found for various $n$-point $d$-dimensional data sets of uniform distributions. Each distribution has a peak at $\sim0$ (indicating the frequency with which the model is the most suitable choice, or at least very nearly the most suitable choice) and a long negatively skewed tail. We see here that the model defined by a linear combination of the beta and uniform distributions is most likely to be the most suitable of these models for the purpose of describing the prominences of noisy subgroups.}
    \label{fig:relative_likelihood}
\end{figure}
